Generative Style Transfer for MRI Image Segmentation: A Case of Glioma Segmentation in Sub-Saharan Africa

In Sub-Saharan Africa (SSA), the utilization of lower-quality Magnetic Resonance Imaging (MRI) technology raises questions about the applicability of machine learning methods for clinical tasks. This study aims to provide a robust deep learning-based brain tumor segmentation (BraTS) method tailored for the SSA population using a threefold approach. Firstly, the impact of domain shift from the SSA training data on model efficacy was examined, revealing no significant effect. Secondly, a comparative analysis of 3D and 2D full-resolution models using the nnU-Net framework indicates similar performance of both the models trained for 300 epochs achieving a five-fold cross-validation score of 0.93. Lastly, addressing the performance gap observed in SSA validation as opposed to the relatively larger BraTS glioma (GLI) validation set, two strategies are proposed: fine-tuning SSA cases using the GLI+SSA best-pretrained 2D fullres model at 300 epochs, and introducing a novel neural style transfer-based data augmentation technique for the SSA cases. This investigation underscores the potential of enhancing brain tumor prediction within SSA's unique healthcare landscape.

==> Tikz/stylizedimages.tex <==


\tikzset{every picture/.style={line width=0.75pt}} %set default line width to 0.75pt        

\begin{tikzpicture}[x=0.75pt,y=0.75pt,yscale=-1,xscale=1]
%uncomment if require: \path (0,300); %set diagram left start at 0, and has height of 300

%Image [id:dp8070261961795717] 
\draw (604,122.35) node  {\includegraphics[width=115.5pt,height=120.53pt]{Stylized_Images/stylized-BraTS-SSA-00126-000.png}};
%Image [id:dp9814152918320191] 
\draw (430,122.35) node  {\includegraphics[width=115.5pt,height=120.53pt]{Stylized_Images/stylized-BraTS-SSA-00132-000.png}};
%Image [id:dp17462501741448277] 
\draw (259,122.35) node  {\includegraphics[width=115.5pt,height=120.53pt]{Stylized_Images/stylized-BraTS-SSA-00148-000.png}};
%Image [id:dp9499333198992093] 
\draw (88,122.35) node  {\includegraphics[width=115.5pt,height=120.53pt]{Stylized_Images/stylized-BraTS-SSA-00198-000.png}};




\end{tikzpicture}
